Lie Group Forced Variational Integrator Networks for Learning and Control of Robot Systems

Incorporating prior knowledge of physics laws and structural properties of dynamical systems into the design of deep learning architectures has proven to be a powerful technique for improving their computational efficiency and generalization capacity. Learning accurate models of robot dynamics is critical for safe and stable control. Autonomous mobile robots, including wheeled, aerial, and underwater vehicles, can be modeled as controlled Lagrangian or Hamiltonian rigid-body systems evolving on matrix Lie groups. In this paper, we introduce a new structure-preserving deep learning architecture, the Lie group Forced Variational Integrator Network (LieFVIN), capable of learning controlled Lagrangian or Hamiltonian dynamics on Lie groups, either from position-velocity or position-only data. By design, LieFVINs preserve both the Lie group structure on which the dynamics evolve and the symplectic structure underlying the Hamiltonian or Lagrangian systems of interest. The proposed architecture learns surrogate discrete-time flow maps allowing accurate and fast prediction without numerical-integrator, neural-ODE, or adjoint techniques, which are needed for vector fields. Furthermore, the learnt discrete-time dynamics can be utilized with computationally scalable discrete-time (optimal) control strategies.

==> LieFVIN (arXiv)/tex/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We introduced a new structure-preserving deep learning strategy to learn discrete-time flow maps for controlled Lagrangian or Hamiltonian dynamics on a Lie group, from position-velocity or position-only data. The resulting maps evolve intrinsically on the Lie group and preserve the symplecticity underlying the systems of interest, which allows to generate physically well-behaved long-term predictions based on short-term trajectories data. Learning discrete-time flow maps instead of vector fields yields better prediction without requiring the use of a numerical integrator, neural ODE, or adjoint techniques. The proposed approach can also be combined with discrete-time optimal control strategies, for instance to achieve stabilization and tracking for robot systems on $\text{SE}(3)$. Possible future directions include extensions to multi-link robots and multi-agent  systems (e.g. on $(\text{SE}(3))^n$). 






==> LieFVIN (arXiv)/tex/Evaluation.tex <==
\section{Evaluation}
\label{sec:exp_results}

We now demonstrate our approach to learn and control a planar pendulum and a crazyflie quadrotor. More details about our implementation can be found in Appendix~\ref{appendix: Implementation}, and our Python/PyTorch code is available at    \ \url{https://thaipduong.github.io/LieFVIN/}


\subsection{Pendulum}
\label{subsec:pendulum_so3}
We consider a planar pendulum with dynamics $ \ddot{\varphi} = -15\sin{\varphi} + 3u,$ where $\varphi$ is the angle with respect to its downward position $\varphi = 0$ and $u \in \mathbb{R}$ is a control input. The mass of the pendulum, the potential energy, and input coefficient are given by $m = 1/3$, $U(\varphi) = 5(1-\cos{\varphi})$,  $g(\varphi) = 1$. We collected $\{(\cos{\varphi}, \sin{\varphi}, \dot{\varphi})\}$ data from an OpenAI Gym environment \citep{Zhong2020}. LieFVIN was trained with position-velocity data as described in Algorithm Ia with $\alpha = 0.5$. The forces were specified as $\mathcal{f}_d^{R+} = 0$ and $\mathcal{f}_d^{R-} = g(q)u$, where $g(q)$ is a neural network. 

Figures \ref{fig:pend_exp}(a), (b), (c) show that the LieFVIN model learned the correct inertia matrix $J$, control gain $g(q)$, and potential energy $U$ (up to a constant offset). Without control input, i.e., $\mathcal{f}_d^{R\pm} = 0$, we use the dynamics model learnt from short-term trajectories of $10$ steps of $0.02$s to generate long-term predictions ($2000$ steps, i.e. $40$s). Figure~\ref{fig:pend_exp}(d) shows that the total energy of the learnt system fluctuates but stays close to the ground truth value. The fluctuation comes from the discretization errors in equations \eqref{eq: SE3 discrete H equation 2}-\eqref{eq: SE3 discrete H equation 4} and model errors for the learnt quantities $J$, $U$, and $g(q)$. Note that the $\text{SO}(3)$ constraint errors remain very small, around $10^{-14}$ (see Figure~\ref{fig:pend_exp}(e)). The phase portraits and the learnt dynamics are close to the ground-truth ones, illustrating the ability to generate long-term predictions using the model learnt from short-term data. Meanwhile, a Multilayer Perceptron black-box model, described in Appendix~\ref{appendix: Implementation Pendulum}, struggles to infer the $\text{SO}(3)$ constraints from data (see Figure~\ref{fig:pend_exp}(e)(g)) and is not able to conserve the total~energy~(see Figure~\ref{fig:pend_exp}(d)).


The learnt dynamics model is combined with MPC as described in Section \ref{subsec:control_strategy} to drive the pendulum from downward position $\varphi = 0$ to a stabilized upright position $\varphi^* = \pi$, $\dot{\varphi}^* = 0$, with input constraint $|u| \leq 20$. Figure~\ref{fig:pend_exp}(h) plots the angle $\varphi$, angular velocity $\dot{\varphi}$, and control input $u$, showing that the pendulum is successfully stabilized using the learnt discrete dynamics model. 





\begin{figure}[ht!]	
\vspace{-0.5mm}
\centering
	\includegraphics[width=0.245\textwidth]{fig/pendulum/M_x_all.pdf}
	\includegraphics[width=0.245\textwidth]{fig/pendulum/V_x.pdf}
	\includegraphics[width=0.245\textwidth]{fig/pendulum/g_x.pdf}
	\includegraphics[width=0.245\textwidth]{fig/pendulum/hamiltonian.pdf}
	\put(-428,9.5){\small \textit{(a)}}	
	\put(-317,9.5){\small \textit{(b)}}
	\put(-206,9.5){\small \textit{(c)}}	
	\put(-95,9.5){\small \textit{(d)}}
			
	\includegraphics[width=0.245\textwidth]{fig/pendulum/SO3_constraints.pdf}
	\includegraphics[width=0.245\textwidth]{fig/pendulum/phase_portrait.pdf}
	\includegraphics[width=0.245\textwidth]{fig/pendulum/loss_log.pdf}
		\includegraphics[width=0.245\textwidth]{fig/pendulum/control.pdf}
	\put(-420,58){\small \textit{(e)}}	
	\put(-315.5,67){\small \textit{(f)}}
	\put(-190,67){\small \textit{(g)}}	
	\put(-97.6,67){\small \textit{(h)}}

\vspace*{-3mm}	
\caption{Evaluation of $\text{SO}(3)$ LieFVIN on a pendulum. We learned the inertia matrix~(a), potential energy~(b), and input coefficient~(c), with the loss function shown in~(g). The learnt model respects the energy conservation law~(d), $\text{SO}(3)$ constraints~(e), and phase portraits~(f). The control from MPC is shown in (h). Meanwhile, a black-box model struggles to infer the $\text{SO}(3)$ constraints from data (e)(g) and is not able to conserve energy (d). }
\label{fig:pend_exp} \vspace*{-1mm}	
\end{figure}	






\subsection{Crazyflie Quadrotor}

We demonstrate that our $\text{SE}(3)$ dynamics learning and control approach can achieve trajectory tracking for an under-actuated system by considering a Crazyflie quadrotor simulated using PyBullet \citep{gym-pybullet-drones2020}. The control input $\bfu = [f, \bftau]$ includes the thrust $f\in \mathbb{R}_{\geq 0}$ and torque vector $\bftau \in \mathbb{R}^3$ generated by the $4$ rotors. LieFVIN is trained as in Algorithm Ib with $\alpha = 0.5$. The forces are specified as $\mathcal{f}_d^{x\pm} = 0.5g_x(q)u$ and $\mathcal{f}_d^{R\pm} = 0.5g_R(q)u$ where $g_x(q),  g_R(q)$ are neural networks. 

Figures \ref{fig:quad_exp}(a)-(e) show that LieFVIN learned the correct mass~$m$, inertia matrix~$J$, control gains~$g_x(q)$ and~$g_R(x)$, and potential energy~$U(q)$ (up to a constant offset). Without control input, i.e., $\mathcal{f}_d^{R\pm} = 0$, we use the dynamics model learnt from short-term trajectories of $5$ steps of $0.02$s to generate long-term predictions ($2000$ steps, i.e. $40$s). Figure~\ref{fig:quad_exp}(f) shows that the total energy of the system has bounded fluctuations while $\text{SO}(3)$ constraint errors are around~$10^{-14}$, verifying the near-energy conservation and manifold constraints guaranteed by our approach.

The learnt model is then combined with MPC as in Section \ref{subsec:control_strategy} to track a diamond-shaped trajectory, with control input constraints $0\leq f \leq 0.595, \  \vert \tau \vert \leq 10^{-3}[5.9 \ \ 5.9 \ \ 7.4 ]^\top$. Figure~\ref{fig:tracking_viz} displays the robot trajectory and plots the tracking errors over time, showing that the quadrotor successfully completes the task.


\begin{figure}[ht!]		
\centering
	\includegraphics[width=0.245\textwidth]{fig/quadrotor/M_x_1.pdf}
        \includegraphics[width=0.245\textwidth]{fig/quadrotor/M_x_2.pdf}
	\includegraphics[width=0.245\textwidth]{fig/quadrotor/g_x.pdf}
        \includegraphics[width=0.245\textwidth]{fig/quadrotor/g_w.pdf}
	\put(-425,8){\small \textit{(a)}}	
	\put(-311,8){\small \textit{(b)}}
	\put(-205,8){\small \textit{(c)}}	
	\put(-96,8){\small \textit{(d)}}
		
	
        \includegraphics[width=0.245\textwidth]{fig/quadrotor/V_x.pdf}
	\includegraphics[width=0.245\textwidth]{fig/quadrotor/hamiltonian.pdf}
	\includegraphics[width=0.245\textwidth]{fig/quadrotor/SO3_constraints.pdf}
	\includegraphics[width=0.245\textwidth]{fig/quadrotor/loss_log.pdf}
	\put(-420,67){\small \textit{(e)}}	
	\put(-311,67){\small \textit{(f)}}
	\put(-201.5,67){\small \textit{(g)}}	
	\put(-90,67){\small \textit{(h)}}

\vspace{-4.1mm}	
\caption{LieFVIN learns the correct mass $m$~(a), inertia matrix $J$~(b), input coefficients $g_x(q)$~(c) and $g_R(q)$~(d), potential energy $U(q)$~(e). The learnt model respects the energy conservation law~(f), $\text{SO}(3)$ constraints~(g). The evolution of the loss function is shown in~(h).}
\label{fig:quad_exp}
\end{figure}	
\begin{figure}[ht!]	
\vspace{-2.5mm}	
\centering
\includegraphics[width=0.73\textwidth]{fig/quadrotor/tracking_results.pdf}
 \hfill
         \begin{minipage}[h]{0.26\textwidth}
         \vspace{-6.1cm}
         \centering
        \includegraphics[width=0.83\textwidth]{fig/quadrotor/crazyflie.png}
        \includegraphics[width=0.93\textwidth]{fig/quadrotor/mpc_traj.pdf}

        \end{minipage}
        
\vspace{-4.2mm}	
\caption{Trajectory tracking with the learned quadrotor model. The tracking errors (left) between reference trajectory (orange) and the actual trajectory, and the robot trajectory (lower right) show that the task is completed successfully.} 
\label{fig:tracking_viz}  
\end{figure}

\newpage 


==> LieFVIN (arXiv)/tex/Introduction.tex <==

\section{Introduction} \label{sec:intro}

Dynamical systems evolve according to physics laws which can be described using differential equations. An accurate model of the dynamics of a control system is important, not only for predicting its future behavior, but also for designing control laws that ensure desirable properties such as safety, stability, and generalization to different operational conditions. 

This paper considers the problem of learning dynamics: given a dataset of trajectories from a dynamical system, we wish to infer the update map that generates these trajectories and use it to predict the evolution of the system from different initial states. Models obtained from first principles are used extensively in practice but tend to over-simplify the underlying structure of dynamical systems, leading to prediction errors that cannot be corrected by optimizing over a few model parameters. Deep learning provides very expressive models for function approximation but standard neural networks struggle to learn the symmetries and conservation laws underlying dynamical systems, and as a result do not generalize well. Deep learning models capable of learning and generalizing dynamics effectively \citep{Willard2020} are typically over-parameterized and require large datasets and substantial training time, making them prohibitively expensive for applications such as robotics. 

  

A recent research direction has been considering a hybrid approach, which encodes physical laws and geometric properties of the underlying system in the design of the neural network architecture or in the learning process. Prior physics knowledge can be used to construct physics-informed neural networks with improved design and efficiency and better generalization capacity, which take advantage of the function approximation power of neural networks to handle incomplete knowledge. In this paper, we consider learning controlled Lagrangian or Hamiltonian dynamics on Lie groups while preserving the symplectic structure underlying these systems and the Lie group constraints. 

Symplectic maps possess numerous special properties and are closely related to Hamiltonian systems. Preserving the symplectic structure of a Hamiltonian system when constructing a discrete approximation of its flow map ensures the preservation of many aspects of the system such as total energy, and leads to physically well-behaved discrete solutions~\citep{LeRe2005,HaLuWa2006,Holm2009,Blanes2017}. It is thus important to have structure-preserving architectures which can learn flow maps and ensure that the learnt maps are symplectic. Many physics-informed approaches have recently been proposed to learn Hamiltonian dynamics and symplectic maps \citep{Lutter2018,Greydanus2019,Bertalan2019,Jin2020,BurbyHenon,Chen2020,Cranmer2020,Zhong2020,zhong2020dissipative,Zhong2021,Marco2021,Rath2021,Chen2021neural,Offen2022,Santos2022,Valperga2022,Mathiesen2022,DuruisseauxNPMap}.

Our physics-informed strategy, inspired by (Forced) Variational Integrator Networks ((F)VINs) \citep{Saemundsson2020,Havens2021}, differs from most of these approaches by learning a discrete-time symplectic approximation to the flow map of the dynamical system, instead of learning the vector field for the continuous-time dynamics. This allows fast prediction for simulation, planning and control without the need to integrate differential equations or use neural ODEs and adjoint techniques. Additionally, the learnt discrete-time dynamics can be combined with computationally scalable discrete-time control strategies. 

The novelty of our approach with respect to (F)VINs resides in the enforcement not only of the preservation of symplecticity but also of the Lie group structure when learning a surrogate map for a controlled Lagrangian system which evolves on a Lie group. This is achieved by working in Lie group coordinates instead of Euclidean coordinates, by matching the training data to a parameterized forced Lie group variational integrator which evolves intrinsically on the Lie group. More specifically, we extend the discrete-time Euclidean formulation of FVINs with control from \citep{Havens2021} to Lie groups in a structure-preserving way, which is particularly relevant when considering robot systems (e.g., wheeled, aerial, and underwater vehicles) since they can often be modeled as controlled Lagrangian rigid-body systems evolving on Lie groups.


Given a learnt dynamical system, it is often desirable to control its behavior to achieve stabilization, tracking, or other control objectives. Control designs for continuous-time Hamiltonian systems rely on the Hamiltonian structure \citep{lutter2019deepunderactuated,Zhong2020, duong21hamiltonian, duong2022adaptive}. Since the Hamiltonian captures the system energy, control techniques for stabilization inject additional energy into the system via the control input to ensure that the minimum of the total energy is at a desired equilibrium. For fully-actuated Hamiltonian systems, it is sufficient to shape the potential energy only using energy-shaping and damping-injection (ES-DI) \citep{van2014port}. For under-actuated systems, both the kinetic and potential energies are shaped, e.g., via interconnection and damping assignment passivity-based control (IDA-PBC) \citep{ortega2002stabilization,van2014port,acosta2014robust,cieza2019ida}. The most widely used control approach for discrete-time dynamics is based on Model Predictive Control (MPC) \citep{borrelli_MPC_book,NMPC_book}. MPC techniques determine an open-loop control sequence that solves a finite-horizon optimal control problem, apply the first few control inputs, and repeat the process. A key result in MPC is that an appropriate choice of terminal cost and terminal constraints in the sequence of finite-horizon problems can guarantee recursive feasibility and asymptotic optimality with respect to the infinite-horizon cost \citep{borrelli_MPC_book}. The ability to learn a structure-preserving discrete-time model of a dynamics system enabled by this paper, also allows employing MPC techniques for optimal control of the learnt system dynamics.

==> LieFVIN (arXiv)/tex/Preliminaries.tex <==


\section{Preliminaries}
\label{sec:prelim}

We first review the basic theory of continuous-time Lagrangian and Hamiltonian systems, before describing their underlying symplectic structure and how variational integrators preserve that structure. Finally, we discuss how external forcing and control can be added to variational integrators.

\subsection{Geometric Mechanics}
The set of tangent vectors to a manifold $\mathcal{Q} $ at a point $q\in \mathcal{Q}$ is a vector space called the tangent space $T_q \mathcal{Q}$ to $\mathcal{Q}$ at $q$. The disjoint union of all the tangent spaces to $\mathcal{Q}$ forms the tangent bundle $T\mathcal{Q} = \{  (q,v) | q\in \mathcal{Q}, v \in T_q\mathcal{Q}  \}$ of $\mathcal{Q}$.  The vector space dual to the tangent space $T_q \mathcal{Q}$ is the cotangent space $T_q^* \mathcal{Q}$, and the vector bundle over $\mathcal{Q}$ whose fibers are the cotangent spaces of $\mathcal{Q}$ is the cotangent bundle $T^*\mathcal{Q}  = \{  (q,p) | q\in \mathcal{Q}, p \in T^*_q \mathcal{Q} \}$. 


Given a manifold $\mathcal{Q} $, a Lagrangian is a function $L:T\mathcal{Q}  \rightarrow \mathbb{R}$. Hamilton's Variational Principle states that $ \delta \int_{0}^{T}{L(q(t),\dot{q}(t))dt} = 0$, where the variation is induced by an infinitesimal variation $\delta q$ that vanishes at the endpoints. Hamilton's Principle is equivalent to the Euler--Lagrange equations
%
\begin{equation}\label{eq: EL Basic}
 \frac{\partial L }{\partial q}(q,\dot{q}) -	\frac{d}{dt} \left( \frac{\partial L} {\partial \dot{q}} (q,\dot{q}) \right) = 0.
\end{equation}
%
Given a Lagrangian $L$, we define the conjugate momentum $p \in T^* \mathcal{Q}$ via the Legendre transform $p = \frac{\partial L}{\partial \dot{q}}$, and obtain a Hamiltonian  $H(q,p) = \sum_{j=1}^{n} {p_j  \dot{q}^j} - L(q,\dot{q})\big|_{p_i=\frac{\partial L}{\partial \dot{q}^i}}$ on $T^*\mathcal{Q}$. There is a variational principle on the Hamiltonian side which is equivalent to Hamilton's equations and to the Euler--Lagrange equations~\eqref{eq: EL Basic} when the Legendre transform is diffeomorphic. For most mechanical systems, the Legendre transform is diffeomorphic and thus the Lagrangian and Hamiltonian formulations are equivalent. The approaches presented here are based on the Lagrangian formulation, but also apply to the equivalent Hamiltonian systems whenever they are well-defined.

\subsection{Symplecticity}

A smooth mapping $(q,p) \mapsto (\bar{q},\bar{p})$ is symplectic if it preserves the symplectic two-form, that is $\sum_{i=1} \mathbf{d}q^i\wedge \mathbf{d}p_i = \sum_{i=1} \mathbf{d}\bar{q}^i\wedge \mathbf{d}\bar{p}_i$. Hamiltonian systems and symplectic flows are closely related: solutions to Hamiltonian systems are symplectic flows \citep{Poincare1899}, and symplectic flows are locally Hamiltonian. When applied to Hamiltonian systems, symplectic integrators yield discrete approximations of the flow that preserve the symplectic two-form, which results in the preservation of many qualitative aspects of the dynamical system and leads to physically well-behaved solutions. See \citep{LeRe2005,HaLuWa2006,Blanes2017} for a comprehensive presentation of geometric numerical integration.




\subsection{Variational Integrators}

 Variational integrators are obtained by discretizing Hamilton's principle, instead of discretizing the equations of motion, are thus symplectic, preserve many invariants, and exhibit excellent long-time near-energy preservation~\citep{MaWe2001}. The exact discrete Lagrangian generating the time-$h$ flow can be represented in boundary-value form as $L_d^E(q_0,q_1)=\int_0^h L(q(t),\dot q(t)) dt ,$ where $q(t)$ satisfies the Euler--Lagrange equations on $[0,h]$ with $q(0)=q_0$, $q(h)=q_1$. After constructing an approximation $L_d$ to $L_d^E$, the Lagrangian variational integrator is defined implicitly by the discrete Euler--Lagrange equation, $D_2 L_d(q_{k-1} , q_k) + D_1 L_d(q_k, q_{k+1})  = 0,$ which can also be written in Hamiltonian form, using discrete momenta $p_k$, as $
	p_k=-D_1 L_d(q_k, q_{k+1})$ and $ p_{k+1}=D_2 L_d(q_k, q_{k+1})$,  
where $D_i$ denotes a partial derivative with respect to the $i$-th argument. Many properties of the integrator, such as momentum conservation and error analysis guarantees, can be determined by analyzing the discrete Lagrangian, instead of analyzing the integrator directly. 

Examples of variational integrators include Taylor~\citep{ScShLe2017}, Galerkin~\citep{MaWe2001,LeZh2011}, prolongation-collocation~\citep{LeSh2011}, and constrained~\citep{MaWe2001,Duruisseaux2022Constrained} variational integrators. Variational integrators can also be developed for Hamiltonian dynamics \citep{LaWe2006, LeZh2011,ScLe2017,duruisseaux2020adaptive}, and can be used with prescribed variable time-steps \citep{duruisseaux2020adaptive,Duruisseaux2022Lagrangian}.

\subsection{Forced Variational Integrators}

External forcing and control can be added to variational integrators \citep{MaWe2001,Ober2011}. Let $u(t)$ be the control parameter in some control manifold $\mathcal{U}$, and consider a Lagrangian control force $\mathcal{f}_L : T\mathcal{Q} \times \mathcal{U} \rightarrow T^* \mathcal{Q}$. Hamilton's principle can be modified into the Lagrange--d'Alembert Principle
\begin{equation} \label{eq: Lagrange dAlembert}
    \delta \int_{0}^{T}{L(q(t),\dot{q}(t))dt} + \int_0^T{\mathcal{f}_L(q(t),\dot{q}(t),u(t)) \cdot \delta q(t) dt} =0,
\end{equation} 
where the variation is induced by an infinitesimal variation $\delta q$ that vanishes at the endpoints. This variational principle is equivalent to the forced Euler--Lagrange equations
\begin{equation}\label{eq: EL Forced}
 \frac{\partial L }{\partial q}(q,\dot{q}) -	\frac{d}{dt} \left( \frac{\partial L} {\partial \dot{q}} (q,\dot{q}) \right) + \mathcal{f}_L(q,\dot{q},u) = 0.
\end{equation}
Using a discrete Lagrangian $L_d$, and discrete Lagrangian control forces $\mathcal{f}_d^{\pm} : \mathcal{Q} \times \mathcal{Q} \times \mathcal{U} \rightarrow T^* \mathcal{Q}$ to approximate the virtual work of the Lagrangian control force $\mathcal{f}_L$,
\begin{equation}
    \int_{t_k}^{t_{k+1}}{\mathcal{f}_L(q(t),\dot{q}(t),u(t)) \cdot \delta q(t) dt} \approx  \mathcal{f}_d^-(q_k,q_{k+1},u_k) \cdot \delta q_k +  \mathcal{f}_d^+(q_k,q_{k+1},u_k)\cdot \delta q_{k+1},
\end{equation}
one can obtain a forced variational integrator from the forced discrete Euler--Lagrange equations
\begin{equation}
	   D_2 L_d(q_{k-1} , q_k)  + D_1 L_d(q_k, q_{k+1}) + \mathcal{f}_d^{+}(q_{k-1},q_k, u_{k-1}) + \mathcal{f}_d^{-}(q_k, q_{k+1},u_k) = 0,
	\end{equation}
which can also be written in Hamiltonian form as
\begin{align}
	p_k  =-D_1 L_d(q_k, q_{k+1}) - \mathcal{f}_d^-(q_k,q_{k+1},u_k), \quad  p_{k+1} =D_2 L_d(q_k, q_{k+1}) + \mathcal{f}_d^+(q_k,q_{k+1},u_k). \label{IDEL-Forced}
\end{align}

==> LieFVIN (arXiv)/tex/ProblemStatement.tex <==
\section{Problem Statement}
\label{sec: problem statement}

We consider the problem of learning controlled Lagrangian dynamics. Given a position-velocity dataset of trajectories, we wish to infer the flow map generating these trajectories, while preserving the system's symplectic structure and constraining the updates to the Lie group on which it evolves. For example, a rigid-body robot system may be modeled as a Lagrangian system evolving on the Lie group $\text{SE}(3)$ of rigid-body transformations. Learning its dynamics from trajectory data should respect kinematic and energy conservation. More precisely, we consider the following problem. \vspace{-2mm}


\begin{problem} \label{problem1}
 Let $\mathcal{Q}$
 be a Lie group and $\mathcal{D}_{T \mathcal{Q}}$ be a distance metric on $T \mathcal{Q}$. Given a dataset of position-velocity updates $\left\{ \left(q_0^{(i)}, \dot{q}_0^{(i)}, u_0^{(i)}\right) \mapsto \left(q_1^{(i)}, \dot{q}_1^{(i)}\right)  \right\}_{i=1}^{N}$ for a controlled Lagrangian dynamical system evolving on $\mathcal{Q}$, we wish to find a symplectic mapping $\Psi : T \mathcal{Q}  \times \mathcal{U} \rightarrow T\mathcal{Q} $ which minimizes  \vspace{-0.5mm}
 %
 \begin{equation}
     \sum_{i=1}^{N}{\mathcal{D}_{T \mathcal{Q}}\left(\left(q_1^{(i)}, \dot{q}_1^{(i)}\right) , \Psi\left(q_0^{(i)}, \dot{q}_0^{(i)}, u_0^{(i)}\right) \right)}.  \vspace{-0.4mm}
 \end{equation}  
 

\end{problem}



==> LieFVIN (arXiv)/tex/TechnicalApproach.tex <==

\section{Lie group Forced Variational Integrators Networks (LieFVINs)}
\label{sec:technical_approach}


To solve Problem \ref{problem1}, we introduce Lie group Forced Variational Integrators Networks (\textcolor{blue}{\textbf{LieFVINs}}). Our main idea is to parametrize the updates of a forced Lie group variational integrator and match them with observed updates. We focus on specific forced $\text{SO}(3)$ and $\text{SE}(3)$ variational integrators, but the general strategy extends to any Lie group forced variational integrator. 


\subsection{The $\text{SO}(3)$ and $\text{SE}(3)$ Lie Groups}

The 3-dimensional special orthogonal group $\text{SO}(3) = \{ R \in \mathbb{R}^{3\times 3} | RR^\top = \mathbb{I}_3, \det{(R)} = 1 \}$, where $\mathbb{I}_k $ denotes the $k \times k$ identity matrix, is the Lie group of rotations about the origin in $\mathbb{R}^3$. The Lie algebra  of $\text{SO}(3)$ is the space of skew-symmetric matrices $\mathfrak{so}(3) = \{ A \in \mathbb{R}^{3\times 3} |  A^\top  = -A \},$
with the matrix commutator $[A,B] = AB-BA$ as the Lie bracket. The sets $\mathbb{R}^{3} $ and $ \mathfrak{so}(3)$ are isomorphic via the hat map $S(\cdot) : \mathbb{R}^{3} \rightarrow \mathfrak{so}(3) $, defined by $S(x) y = x\times y$ for any $ x,y\in \mathbb{R}^3$. 

The Special Euclidean group in 3 dimensions, $\text{SE}(3)$, is a semidirect product of $\mathbb{R}^3$ and $\text{SO}(3)$ and is diffeomorphic to $\mathbb{R}^3 \times \text{SO}(3)$. Elements of $\text{SE}(3)$ can be written as $(x,R) \in \mathbb{R}^3 \times \text{SO}(3)$, and the Lie algebra $\mathfrak{se}(3)$ of $\text{SE}(3)$ is composed of elements $(y,A) \in \mathbb{R}^3 \times \mathfrak{so}(3)$. 

The pose of a rigid body can be described by an element $(x,R)$ of $\text{SE}(3)$, consisting of position $x \in \bbR^3$ and orientation $R \in \text{SO}(3)$. See Appendix~\ref{appendix: Rigid-Body Kinematics} for more details about rigid-body kinematics.


\subsection{Forced Variational Integrator on $\text{SO}(3)$ and $\text{SE}(3)$}  \label{sec: Variational Integrator}

On $\text{SE}(3)$, $q = (x,R)$ and $\dot{q} = (v,\omega)$ where $x$ is position, $R$ is orientation, $v$ is velocity, and $\omega$ is angular velocity. A Lagrangian on $\text{SE}(3)$ is given by \vspace{-1mm}
%
\begin{equation} 
L(x,R,v,\omega) = \frac{1}{2} v^\top mv  +\frac{1}{2} \omega^\top  J \omega  - U(x,R),  
\end{equation}  
%
where $m$ is mass, $J \in \mathbb{R}^{3\times 3}$ is a symmetric positive-definite inertia matrix, $U$ is potential energy. \\


Consider the continuous-time kinematics equation $\dot{R} = RS(\omega)$, with constant $\omega(t) \equiv \omega_k$ for a short period of time $t \in [t_k,t_{k+1})$ where $t_{k+1} = t_k + h$. Then, $R(t_{k+1}) = R(t_k)\exp(h S(\omega_k))$. Thus, with $R_k := R(t_k)$, $R_{k+1} := R(t_{k+1})$ and $Z_k := \exp(h S(\omega_k))$, we obtain $R_{k+1} = R_k Z_k$ and for sufficiently small $h$, we have $Z_k \approx \mathbb{I}_3 + h S(\omega_k)$. With $(x_k,R_k) \in \text{SE}(3)$, the discrete $\text{SE}(3)$ kinematic equations are given by $R_{k+1} = R_k Z_k$ and $x_{k+1} = x_k +R_k y_k$ where $ (y_k, Z_k)\in \text{SE}(3)$, which ensures that the sequence of updates $\{(x_k, R_k) \}_k$ remains on $\text{SE}(3)$. 

Using the approximation $S(\omega_k) \approx \frac{1}{h} ( Z_k - \mathbb{I}_3 )$, we choose the discrete Lagrangian
%
\begin{equation}  \label{eq: discrete Lagrangian}
\begin{aligned}
L_d(x_k, R_k, y_k, Z_k  )  &  =  \frac{m}{2h} y_k^\top y_k + \frac{1}{h} \text{tr}\left( [\mathbb{I}_3  - Z_k] J_d \right)  \\ &  \qquad \quad - (1-\alpha ) h U(x_k, R_k) - \alpha  h  U(x_k + R_ky_k, R_k Z_k),
\end{aligned}
\end{equation} 
%
where $\alpha \in [0,1]$ and $J_d = \frac{1}{2} \text{tr}(J) \mathbb{I}_3 - J$. Equation~\eqref{eq: discrete Lagrangian} gives a simple approximation to the exact $\text{SE}(3)$ discrete Lagrangian, while maintaining some flexibility in the two-point quadrature weights through the tunable parameter $\alpha$. Higher-order approximations could also be used, but the resulting discrete equations of motion would typically be more complicated and expensive to evolve. 

We denote $U_k = U(x_k,R_k)$ and define $\xi_k$ via $ S(\xi_k) = \frac{\partial  U_{k}}{\partial R_{k}}^\top R_{k} - R_{k}^\top \frac{\partial U_{k}}{\partial R_{k}}$. In Appendix~\ref{appendix: Derivation of integrator}, we show that the forced discrete Euler--Lagrange equations associated to the discrete Lagrangian~\eqref{eq: discrete Lagrangian} and discrete control forces $\mathcal{f}_{d_k}^{\pm} \equiv \mathcal{f}_{d}^{\pm}(x_k, R_k, u_k)$ with $R$ and $x$ components $\mathcal{f}_{d}^{R\pm},\mathcal{f}_{d}^{x\pm}$ can be written in Hamiltonian form, using $\pi_k = J \omega_k  $ and $\gamma_k = m v_k $, as
%
\begin{align}
   & hS(\pi_k)   +   h S( \mathcal{f}_{d_k}^{R-}) + (1-\alpha)h^2 S(\xi_k)  =  Z_k J_d - J_d Z_k^\top    \label{eq: SE3 discrete H equation 2}, \\ &
    R_{k+1}  = R_k Z_k  \label{eq: SE3 discrete H equation 5} , \\
    & \pi_{k+1}  = Z_k^\top \pi_k + (1-\alpha)h Z_k^\top \xi_k+ \alpha h \xi_{k+1}   + Z_k^\top \mathcal{f}_{d_k}^{R-}+ \mathcal{f}_{d_k}^{R+}   \label{eq: SE3 discrete H equation 1}, \\ &
      x_{k+1}  =  x_{k} + \frac{h}{m} \gamma_k - (1-\alpha)\frac{h^2}{m} \frac{\partial U_k}{\partial x_k} -  \frac{h}{m} R_k \mathcal{f}_{d_k}^{x-}  \label{eq: SE3 discrete H equation 3}, \\ &
        \gamma_{k+1}  = \gamma_k - (1-\alpha)h    \frac{\partial U_k}{\partial x_k} - \alpha h \frac{\partial U_{k+1}}{\partial x_{k+1}} +  R_k \mathcal{f}_{d_k}^{x-} + R_{k+1} \mathcal{f}_{d_k}^{x+}   \label{eq: SE3 discrete H equation 4}.
\end{align}
%
Given $(x_k,R_k,\gamma_k, \pi_k, u_k)$, we first solve equation \eqref{eq: SE3 discrete H equation 2} which is of the form $S(a) = Z J_d  - J_d Z^\top$ as outlined in Remark~\ref{remark: Cayley}, and then get $R_{k+1} = R_k Z_k$. We then obtain $\pi_{k+1}$,  $x_{k+1}$ and $\gamma_{k+1}$ from equations~\eqref{eq: SE3 discrete H equation 1}-\eqref{eq: SE3 discrete H equation 4}. The discrete equations of motion can be rewritten as an update from $(x_k,  R_k, v_k,\omega_k, u_k)$ to $(x_{k+1}, R_{k+1}, v_{k+1}, \omega_{k+1})$ by using $\pi_k = J \omega_k  $ and $\gamma_k = m v_k $.  



\begin{remark}\label{remark: Cayley}  $ S(a) = Z J_d  - J_d Z^\top$ can be converted into an equivalent vector equation 
\begin{equation} \label{eq: Vector Equation General Form}
   \phi(\mathcal{z}) \equiv a + a \times \mathcal{z} + \mathcal{z}(a^\top \mathcal{z}) - 2J\mathcal{z} = 0, \qquad  \mathcal{z}\in \mathbb{R}^3,
\end{equation}
as shown in Appendix~\ref{appendix: Equation Transformation}, using the Cayley transform 
\begin{equation} Z = \text{Cay}(\mathcal{z}) \equiv  (\mathbb{I}_3+S(\mathcal{z}))(\mathbb{I}_3-S(\mathcal{z}))^{-1} = \frac{1}{1+ \| \mathcal{z} \|_2^2}\left((1-\| \mathcal{z} \|_2^2) \mathbb{I}_3 + 2 S(\mathcal{z}) + 2 \mathcal{z} \mathcal{z}^\top \right). \vspace{-0.55mm} \end{equation}


The solution $Z=\text{Cay}(\mathcal{z})$ to the original equation $ S(a) = Z J_d  - J_d Z^\top$ can be obtained after solving this vector equation for $\mathcal{z}$ by using (typically 2 or 3 steps of) Newton's method:
\begin{equation}
    \mathcal{z}^{(n+1)} = \mathcal{z}^{(n)}  - \left[ \nabla \phi (\mathcal{z}^{(n)}) \right]^{-1} \phi (\mathcal{z}^{(n)}), \qquad \nabla \phi(\mathcal{z}) = S(a) + (a^\top \mathcal{z}) \mathbb{I}_3 + \mathcal{z}a^\top - 2J.
\end{equation}

\end{remark}


\vspace{-2mm} 


 \subsection{Lie Group Forced Variational Integrator Networks (LieFVINs) on \text{SE}(3)} \label{sec: Lie Group Variational Integrator Networks}
 
We now describe the construction of Lie group Forced Variational Integrator Networks (\textcolor{blue}{\textbf{LieFVINs}}), for the forced variational integrator on $\text{SE}(3)$ presented in Section~\ref{sec: Variational Integrator}. The idea is to parametrize the updates of the integrator and match them with observed updates. Here, we consider the case where position-velocity data is available, in which case the LieFVIN is based on equations~\eqref{eq: SE3 discrete H equation 2}-\eqref{eq: SE3 discrete H equation 4}. The case where only position data is available is presented in Appendix~\ref{appendix: position only}. 

We parametrize \textcolor{mygreen}{$m$}, $\mathcal{f}_d^{\pm}$ and $U$ as neural networks. The inertia $J$ is a symmetric positive-definite matrix-valued function of $(x,R)$ constructed via a Cholesky decomposition $J = LL^\top $ for a lower-triangular matrix $L$ implemented as a neural network. Given $J$, we also obtain $J_d = \frac{1}{2} \text{tr}(J) \mathbb{I}_3 - J$. To deal with the implicit nature of equation~\eqref{eq: SE3 discrete H equation 2}, we propose two algorithms, based either on an explicit iterative solver or by penalizing deviations away from equation~\eqref{eq: SE3 discrete H equation 2}: \vspace{-2mm} 
 

\noindent \hrulefill

\noindent \textbf{Algorithm Ia.} Given position-velocity data $\{ (\textcolor{mygreen}{x_0}, R_0, \textcolor{mygreen}{v_0},\omega_0, u_0) \mapsto (\textcolor{mygreen}{x_1},  R_1 , \textcolor{mygreen}{v_1}, \omega_1)  \}$, minimize discrepancies between the observed $ (\textcolor{mygreen}{x_1},  R_1, \textcolor{mygreen}{v_1}, \omega_1)$ quadruples and the predicted $(\textcolor{mygreen}{\tilde{x}_1},\tilde{R}_1, \textcolor{mygreen}{\tilde{v}_1}, \tilde{\omega}_1)$ quadruples, obtained as follows: for each $(\textcolor{mygreen}{x_0}, R_0, \textcolor{mygreen}{v_0}, \omega_0, u_0)$ data tuple,
\begin{enumerate}
\item Get $\mathcal{f}^{R \pm}_{d_0}$ \textcolor{mygreen}{and $\mathcal{f}^{x \pm}_{d_0}$} from $(\textcolor{mygreen}{x_0},R_0,u_0)$, and $ \xi_0$ from $ S(\xi_0) = \frac{\partial U_{0}}{\partial R_{0}}^\top R_{0} - R_{0}^\top \frac{\partial U_{0}}{\partial R_{0}}$
    \item Get $Z_0 = \text{Cay}(\mathcal{z})$ where $\mathcal{z}$ is obtained using a few steps of Newton's method to solve the vector equation~\eqref{eq: Vector Equation General Form} equivalent to 
$  h S(J\omega_0)  +  h S( \mathcal{f}_{d_0}^{R-}) + (1-\alpha) h^2 S(\xi_0) = Z J_d - J_d Z^\top$
\item Compute $\tilde{R}_1 = R_0 Z_0$, and then get $\xi_1$ from $ S(\xi_1) = \frac{\partial U_{1}}{\partial \tilde{R}_{1}}^\top \tilde{R}_{1} - \tilde{R}_{1}^\top \frac{\partial U_{1}}{\partial \tilde{R}_{1}}$
\item Get $\tilde{\omega}_1$ from $ J \tilde{\omega}_1 =  Z_0^\top J\omega_0 + (1-\alpha) h Z_0^\top \xi_0 + \alpha h \xi_{1} + Z_0^\top \mathcal{f}_{d_0}^{R-}+ \mathcal{f}_{d_0}^{R+}  $  
\textcolor{mygreen}{ \item  Compute $\begin{bmatrix}  \tilde{x}_1 \\ \tilde{v}_1  \end{bmatrix} = \begin{bmatrix}  x_0 \\ v_0  \end{bmatrix} + \frac{1}{m} \begin{bmatrix}   h m v_0 - (1-\alpha)h^2 m \frac{\partial U_0}{\partial x_0} -   h R_0 \mathcal{f}_{d_0}^{x-} \\  - (1-\alpha) h^2 \frac{\partial U_0}{\partial x_0} - \alpha h^2 \frac{\partial U_1}{\partial x_1}  + R_0 \mathcal{f}_{d_0}^{x-} +  R_1 \mathcal{f}_{d_0}^{x+}  \end{bmatrix}$} \vspace{-0.7mm}
\end{enumerate} \noindent \hrulefill


\noindent \textbf{Algorithm Ib.}  Given position-velocity data $\{ (\textcolor{mygreen}{x_0},  R_0, \textcolor{mygreen}{v_0}, \omega_0, u_0) \mapsto (\textcolor{mygreen}{x_1},  R_1 , \textcolor{mygreen}{v_1}, \omega_1)  \}$, minimize
\begin{itemize}
    \item Discrepancies between the observed $ (\textcolor{mygreen}{x_1}, \textcolor{mygreen}{v_1}, \omega_1)$ triples and the predicted $(\textcolor{mygreen}{\tilde{x}_1}, \textcolor{mygreen}{\tilde{v}_1}, \tilde{\omega}_1)$ triples
    \item Deviations away from the equation $  h S(J\omega_0)  +  h S( \mathcal{f}_{d_0}^{R-}) + (1-\alpha)h^2 S(\xi_0) = J_d Z_0 - Z_0^\top J_d$
\end{itemize}
where, for each $(\textcolor{mygreen}{x_0},  R_0, \textcolor{mygreen}{v_0}, \omega_0, u_0, R_1)$ data tuple,
\begin{enumerate}
     \item $\mathcal{f}^{R \pm}_{d_0}$ \textcolor{mygreen}{and $\mathcal{f}^{x \pm}_{d_0}$} are obtained from $(\textcolor{mygreen}{x_0},R_0,u_0)$, and $ \xi_0,\xi_1$ from $ S(\xi_k) = \frac{\partial U_{k}}{\partial R_{k}}^\top R_{k} - R_{k}^\top \frac{\partial U_{k}}{\partial R_{k}}$
     \item $Z_0 = R_0^\top R_1$ and $\tilde{\omega}_1 = J^{-1}\left[  Z_0^\top J\omega_0 + (1-\alpha)h Z_0^\top \xi_0 + \alpha h \xi_{1} + Z_0^\top \mathcal{f}_{d_0}^{R-}+ \mathcal{f}_{d_0}^{R+} \right] $      \vspace{-0.7mm}       \textcolor{mygreen}{\item  $\begin{bmatrix}  \tilde{x}_1 \\ \tilde{v}_1  \end{bmatrix} = \begin{bmatrix}  x_0 \\ v_0  \end{bmatrix} + \frac{1}{m} \begin{bmatrix}   h m v_0 - (1-\alpha)h^2 m \frac{\partial U_0}{\partial x_0} -   h R_0 \mathcal{f}_{d_0}^{x-} \\  - (1-\alpha) h^2 \frac{\partial U_0}{\partial x_0} - \alpha h^2 \frac{\partial U_1}{\partial x_1}  + R_0 \mathcal{f}_{d_0}^{x-} +  R_1 \mathcal{f}_{d_0}^{x+}  \end{bmatrix}$}  \vspace{-1mm}
\end{enumerate} \noindent \hrulefill


This general strategy extends to any other Lie group integrator. In particular, LieFVINs on $\text{SO}(3)$ can be obtained from the algorithms above as the special case where $x$ is constant, in which case we can disregard all the variables and operations in \textcolor{mygreen}{green}. Lie group variational integrator networks without forces (\textcolor{blue}{\textbf{LieVINs}}) can be obtained by setting $\mathcal{f}_{d_0}^{R\pm} = \mathcal{f}_{d_0}^{x\pm} = 0$. Note that the strategy behind Algorithm Ia enforces the structure of the system in a stronger way than in Algorithm Ib. However, for certain Lie groups and variational integrators, it might not be practical to use Newton's method to solve for the implicit updates, in which case Algorithm Ib is preferred. 






\subsection{Control Strategy}
\label{subsec:control_strategy}

%\hfill 

Given the discrete-time flow map $\Psi$ learnt by a LieFVIN, we can formulate a Model Predictive Control (MPC) problem to design a discrete-time control policy for the dynamical system:  \vspace{-2mm}

\noindent \hrulefill

\noindent At each step $t_\ell  = \ell h$,
\begin{enumerate}
    \item Obtain an estimate $(\tilde{q}_\ell , \dot{\tilde{q}}_\ell)$ of the current state.
    
    \item Solve a $N$-step finite horizon optimal control problem starting at $(\tilde{q}_\ell , \dot{\tilde{q}}_\ell)$, formulated as a constrained optimization problem: \vspace{-2mm} \textit{Minimize the discrete cost function} 
\begin{equation} \label{eq:mpc problem} \mathcal{J}_d  (U_{\ell}) = \sum_{k =0}^{N-1}{\mathcal{C}_d(q_{\ell+k},q_{\ell+k+1},\dot{q}_{\ell+k},u_{\ell +k})} + \Phi_d(q_{\ell + N-1},q_{\ell +N},\dot{q}_{\ell + N},u_{\ell +N-1} ), \vspace{-1.6mm}
\end{equation}
\textit{over admissible discrete controls} $U_{\ell} = \{u_\ell, u_{\ell +1} , ..., u_{\ell + N-1}  \}$, \textit{subject to path constraints} $
    \mathcal{P}_d(q_{\ell +k},q_{\ell + k+1},\dot{q}_{\ell +k},u_{\ell +k}) \geq  0$  \textit{for }   $k=1,...,N-1$ \textit{and to the termination condition} $\mathcal{T}_d(q_{\ell + N-1},q_{\ell +N},\dot{q}_{\ell +N},u_{\ell + N-1}) = 0,$
\textit{and where the evolution of the controlled system is prescribed by the surrogate symplectic map $\Psi$ learnt by the LieFVIN.}  
    
    \item Apply the resulting optimal control $u^*_\ell $ to the system in state $(\tilde{q}_\ell , \dot{\tilde{q}}_\ell)$ until $t_{\ell +1} = (\ell +1)h$.
\end{enumerate}  \vspace{-5.2mm}
\noindent \hrulefill

Note that the Lie group constraints do not need to be added as path constraints since they are automatically satisfied to (almost) machine precision, by the design of the LieFVINs. 
In our experiments, we use the PyTorch MPC framework\footnote{Code: \url{https://locuslab.github.io/mpc.pytorch/}} \citep{tassa2014control, amos2018differentiable}.




==> LieFVIN (arXiv)/tex/sym.tex <==
\newcommand{\prl}[1]{\left(#1\right)}
\newcommand{\brl}[1]{\left[#1\right]}
\newcommand{\crl}[1]{\left\{#1\right\}}
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\diag}{diag}
\newcommand{\scaleMathLine}[2][1]{\resizebox{#1\linewidth}{!}{$\displaystyle{#2}$}}

\usepackage{dutchcal}
\newcommand{\bsym}[1]{{\boldsymbol{#1}}}

% Calligraphic fonts
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}

% Fraktur fonts
\newcommand{\frakA}{{\mathfrak{A}}}
\newcommand{\frakB}{{\mathfrak{B}}}
\newcommand{\frakC}{{\mathfrak{C}}}
\newcommand{\frakD}{{\mathfrak{D}}}
\newcommand{\frakE}{{\mathfrak{E}}}
\newcommand{\frakF}{{\mathfrak{F}}}
\newcommand{\frakG}{{\mathfrak{G}}}
\newcommand{\frakH}{{\mathfrak{H}}}
\newcommand{\frakI}{{\mathfrak{I}}}
\newcommand{\frakJ}{{\mathfrak{J}}}
\newcommand{\frakK}{{\mathfrak{K}}}
\newcommand{\frakL}{{\mathfrak{L}}}
\newcommand{\frakM}{{\mathfrak{M}}}
\newcommand{\frakN}{{\mathfrak{N}}}
\newcommand{\frakO}{{\mathfrak{O}}}
\newcommand{\frakP}{{\mathfrak{P}}}
\newcommand{\frakQ}{{\mathfrak{Q}}}
\newcommand{\frakR}{{\mathfrak{R}}}
\newcommand{\frakS}{{\mathfrak{S}}}
\newcommand{\frakT}{{\mathfrak{T}}}
\newcommand{\frakU}{{\mathfrak{U}}}
\newcommand{\frakV}{{\mathfrak{V}}}
\newcommand{\frakW}{{\mathfrak{W}}}
\newcommand{\frakX}{{\mathfrak{X}}}
\newcommand{\frakY}{{\mathfrak{Y}}}
\newcommand{\frakZ}{{\mathfrak{Z}}}

\newcommand{\fraka}{{\mathfrak{a}}}
\newcommand{\frakb}{{\mathfrak{b}}}
\newcommand{\frakc}{{\mathfrak{c}}}
\newcommand{\frakd}{{\mathfrak{d}}}
\newcommand{\frake}{{\mathfrak{e}}}
\newcommand{\frakf}{{\mathfrak{f}}}
\newcommand{\frakg}{{\mathfrak{g}}}
\newcommand{\frakh}{{\mathfrak{h}}}
\newcommand{\fraki}{{\mathfrak{i}}}
\newcommand{\frakj}{{\mathfrak{j}}}
\newcommand{\frakk}{{\mathfrak{k}}}
\newcommand{\frakl}{{\mathfrak{l}}}
\newcommand{\frakm}{{\mathfrak{m}}}
\newcommand{\frakn}{{\mathfrak{n}}}
\newcommand{\frako}{{\mathfrak{o}}}
\newcommand{\frakp}{{\mathfrak{p}}}
\newcommand{\frakq}{{\mathfrak{q}}}
\newcommand{\frakr}{{\mathfrak{r}}}
\newcommand{\fraks}{{\mathfrak{s}}}
\newcommand{\frakt}{{\mathfrak{t}}}
\newcommand{\fraku}{{\mathfrak{u}}}
\newcommand{\frakv}{{\mathfrak{v}}}
\newcommand{\frakw}{{\mathfrak{w}}}
\newcommand{\frakx}{{\mathfrak{x}}}
\newcommand{\fraky}{{\mathfrak{y}}}
\newcommand{\frakz}{{\mathfrak{z}}}

% Sets:
\newcommand{\setA}{\textsf{A}}
\newcommand{\setB}{\textsf{B}}
\newcommand{\setC}{\textsf{C}}
\newcommand{\setD}{\textsf{D}}
\newcommand{\setE}{\textsf{E}}
\newcommand{\setF}{\textsf{F}}
\newcommand{\setG}{\textsf{G}}
\newcommand{\setH}{\textsf{H}}
\newcommand{\setI}{\textsf{I}}
\newcommand{\setJ}{\textsf{J}}
\newcommand{\setK}{\textsf{K}}
\newcommand{\setL}{\textsf{L}}
\newcommand{\setM}{\textsf{M}}
\newcommand{\setN}{\textsf{N}}
\newcommand{\setO}{\textsf{O}}
\newcommand{\setP}{\textsf{P}}
\newcommand{\setQ}{\textsf{Q}}
\newcommand{\setR}{\textsf{R}}
\newcommand{\setS}{\textsf{S}}
\newcommand{\setT}{\textsf{T}}
\newcommand{\setU}{\textsf{U}}
\newcommand{\setV}{\textsf{V}}
\newcommand{\setW}{\textsf{W}}
\newcommand{\setX}{\textsf{X}}
\newcommand{\setY}{\textsf{Y}}
\newcommand{\setZ}{\textsf{Z}}

% Vectors
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}


\newcommand{\bfalpha}{{\boldsymbol{\alpha}}}
\newcommand{\bfbeta}{{\boldsymbol{\beta}}}
\newcommand{\bfgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bfdelta}{{\boldsymbol{\delta}}}
\newcommand{\bfepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bfzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bfeta}{{\boldsymbol{\eta}}}
\newcommand{\bftheta}{{\boldsymbol{\theta}}}
\newcommand{\bfiota}{{\boldsymbol{\iota}}}
\newcommand{\bfkappa}{{\boldsymbol{\kappa}}}
\newcommand{\bflambda}{{\boldsymbol{\lambda}}}
\newcommand{\bfmu}{{\boldsymbol{\mu}}}
\newcommand{\bfnu}{{\boldsymbol{\nu}}}
\newcommand{\bfomicron}{{\boldsymbol{\omicron}}}
\newcommand{\bfpi}{{\boldsymbol{\pi}}}
\newcommand{\bfrho}{{\boldsymbol{\rho}}}
\newcommand{\bfsigma}{{\boldsymbol{\sigma}}}
\newcommand{\bftau}{{\boldsymbol{\tau}}}
\newcommand{\bfupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\bfphi}{{\boldsymbol{\phi}}}
\newcommand{\bfchi}{{\boldsymbol{\chi}}}
\newcommand{\bfpsi}{{\boldsymbol{\psi}}}
\newcommand{\bfomega}{{\boldsymbol{\omega}}}
\newcommand{\bfxi}{{\boldsymbol{\xi}}}
\newcommand{\bfell}{{\boldsymbol{\ell}}}

% Matrices
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}


\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\bfDelta}{\boldsymbol{\Delta}}
\newcommand{\bfTheta}{\boldsymbol{\Theta}}
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}
\newcommand{\bfPi}{\boldsymbol{\Pi}}
\newcommand{\bfSigma}{\boldsymbol{\Sigma}}
\newcommand{\bfUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bfPhi}{\boldsymbol{\Phi}}
\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfOmega}{\boldsymbol{\Omega}}


% Blackboard Bold:
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}





% Environments
\newtheorem*{proposition*}{Proposition}
\newtheorem*{corollary*}{Corollary}
%\theoremstyle{definition}
\newtheorem{assumption}{Assumption} 
\newtheorem*{assumption*}{Assumption}
\newtheorem*{problem*}{Problem}
\newtheorem{problem}{Problem}
%\theoremstyle{remark}
\newtheorem*{solution*}{Solution}
\newtheorem*{remark*}{Remark}

